LMPriors: Pre-Trained Language Models as Task-Specific Priors

Particularly in low-data regimes, an outstanding challenge in machine learning is developing principled techniques for augmenting our models with suitable priors. This is to encourage them to learn in ways that are compatible with our understanding of the world. But in contrast to generic priors such as shrinkage or sparsity, we draw inspiration from the recent successes of large-scale language models (LMs) to construct task-specific priors distilled from the rich knowledge of LMs. Our method, Language Model Priors (LMPriors), incorporates auxiliary natural language metadata about the task -- such as variable names and descriptions -- to encourage downstream model outputs to be consistent with the LM's common-sense reasoning based on the metadata. Empirically, we demonstrate that LMPriors improve model performance in settings where such natural language descriptions are available, and perform well on several tasks that benefit from such prior knowledge, such as feature selection, causal inference, and safe reinforcement learning.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Section~\ref{discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Section~\ref{discussion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Appendix~\ref{addtl-results}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Appendix~\ref{addtl-results}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{We only used open source datasets for our experiments.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}



==> sections/old_experiments.tex <==
\section{Empirical Evaluations}
\label{experiments}
In this section, we are interested in empirically answering the following questions:
\begin{enumerate}
    \item Is LMPrior a sensible prior? (does it actually contain commonsense knowledge)
    \item Can it be used for downstream tasks such as causal discovery and feature selection?
\end{enumerate}
% \kristy{We will probably also need some (a lot?) of ablation studies on the impact of the prompt design, etc}

% \subsection{Baselines Fail with Limited Data}
% \kristy{we need some kind of demonstration of this, either here or close to the introduction to convince the reader that this is a real problem}

% \subsection{Basic Probability Warm-Up}
% As a warm-up, we empirically verify that LMPrior is able to provide natural language prompt completions which are in accordance with our common sense. 
% Specifically, we experiment with a variety of prompts that test the LM's ability to manipulate and reason about common probability distributions and frequencies of event occurances, such as the likelihood that a 6-sided die will land on 1.
% \kristy{As shown in Figure~\ref{TODO}, we find that LMPrior is indeed able to solve these tasks.}
% For example, \kristy{probability of heads}
% \kristy{do we want something like a warm-up experiment where LMPrior gives us some evidence that it has common sense?}

% \subsection{Multitask Learning}
\subsection{Robustness to Dataset Corruption}
We first evaluate the effectiveness of the feature selection LMPrior $\cP_{\textrm{fs}}$ in a semi-synthetic experiment. 
% LMPrior for working with multiple data sources in a semi-synthetic setting \kristy{TODO: what needs to come out is that LMPrior is being used as a way to filter out irrelevant variables/clean up noisy and corrupted data}.
Specifically, we simulate a dataset corruption setting where a base dataset---which defines the underlying prediction task of interest (e.g. predicting housing prices)---has been contaminated by random Gaussian noise or examples from a secondary, unrelated data source.
% from a mixture from a different data source (or both).
We leverage a wide range of datasets from the UCI Machine Learning repository \citep{asuncion2007uci} such as California Housing Prices, Breast Cancer Detection, Wine Quality, and Adult Census Income, and compare the performance of LMPrior $\cP_{\textrm{fs}}$ across various dataset combinations.
% , and \kristy{XYZ}. \kristy{potential concern: \citep{ding2021retiring} explicitly calls out the Income dataset for being bad haha}
% Another scenario which we simulated was appending features from different datasets like (California Housing Prices, UCI Breast Cancer, UCI Wine dataset, Adult Census Income dataset etc.) to a base dataset. In this set of experiments, we studied
% \begin{itemize}
%     \item Experiment 1: how well LMPrior performed while segregating the features
%     \item Experiment 2: whether the drop in the classification accuracy after corruption (whenever such a drop was observed) could be improved by filtering the fake features out using LMPrior.
% \end{itemize}
% For all experiments, we used OpenAI's \texttt{davinci-instruct-beta} engine to perform the feature selection and classifiers from \texttt{scikit-learn}.

\paragraph{Dataset Separation.} We assess whether the LMPrior $\cP_{\textrm{fs}}$ can successfully filter out the nuisance variables from the original features from the base dataset.
To do so, we leverage the following prompt structure (specialized for the breast cancer prediction task) followed by relevant examples for few-shot learning:

\texttt{A medical institute is trying to use characteristics of the cell
nuclei present in the image as features to
predict whether patients have breast cancer. 
Y means the feature is important for the prediction task, N means
the feature is not important.}

% For few-shot learning \citep{radford2021learning}\kristy{TODO: good few-shot learning citations with GPT}, we provide LMPrior with examples of which features would and would not be useful for the classification task are also added to the prompt. 
% Then we ask the language model whether a feature in our corrupted dataset is important to the prediction task or not, based on its name and description. 
LMPrior is then tasked with responding with a \texttt{Y} or \texttt{N} completion given a variable name and a brief description.
The final importance of a feature is obtained by computing the difference of the log-probabilities
% logits \cc{I think we can say 'log-probabilities' here (ofc it doesn't matter since we're looking at a probability ratio)} 
of the LM identifying the feature as important (\texttt{Y}) vs not important (\texttt{N}):
$$\texttt{score}(\rvc) = \log \lm(\texttt{Y} \vert \rvc) - \log \lm(\texttt{N} \vert \rvc)$$
As shown in Figure~\ref{fig:histo}, LMPrior is able to achieve completion separation of the two disparate feature sets. Interestingly, we find that in cases of no clear separation, the nuisance features which are marked as important by LMPrior are semantically meaningful for the corresponding prediction task.
For example, in Figure~\ref{fig:histo}(e), LMPrior selects two semantically relevant features---gender and age of the person---from the Adult Census Income dataset.
% the two features from Adult Census Income dataset that LMPrior 
% being marked as important for detecting breast cancer are the gender and age of the person.
% shows that this method works really well to select the correct features of the original datasets.
% As shown in \ref{fig:histo},  the base dataset is marked in blue while the dataset which was mixed in is marked in orange. The prompt was always constructed to egg LMPrior to predict features of the base dataset. \kristy{TODO}
\begin{figure*}[!t]
    \centering
        \subfigure[housing-income]{\includegraphics[width=.18\textwidth]{figures/housing-income.png}}
        \subfigure[housing-wine]{\includegraphics[width=.18\textwidth]{figures/housing-wine.png}}
        \subfigure[cancer-housing]{\includegraphics[width=.18\textwidth]{figures/cancer-housing.png}}
        \subfigure[cover-cancer]{\includegraphics[width=.18\textwidth]{figures/covertype_cancer.png}}
        \subfigure[income-cancer]{\includegraphics[width=.18\textwidth]{figures/income-cancer.png}}
    \caption{\kristy{FIX THIS!!!!!!!!!}}
    \label{fig:histo}
\end{figure*}
% \subsubsection*{Experiment 1}
% The prompt starts with a description of the task we are trying to fulfil. In order to do few-shot learning, examples of which features would and would not be useful for the classification task are also added to the prompt. Then we ask the language model whether a feature in our corrupted dataset is important to the prediction task or not, based on its name and description. The final importance assigned to a feature is measured by the difference of log likelihood scores of the LM identifying the feature as important v/s not important. \ref{fig:histo} shows that this method works really well to select the correct features of the original datasets.
% \sanjari{ decide a pattern for plots and use the same for each one}\\
% \begin{figure}[ht!]
%   \centering
%   \includegraphics[width=2in]{figures/housing-income.png}\\
%   \includegraphics[width=2in]{figures/housing-wine.png}\\
%   \includegraphics[width=2in]{figures/cancer-housing.png}\\
%   \includegraphics[width=2in]{figures/covertype_cancer.png}\\
%     \label{fig:histo}
% \end{figure}
% Please note that in such cases, it is possible to revert any drop in classification accuracy after corruption after tuning the feature selection threshold appropriately, because LMPrior manages to separate the features completely.
% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=2in]{figures/income-cancer.png}\\
%     \label{fig:cancer-income}
% \end{figure}

\kristy{TODO: PLOT SHOWING THE EFFECT OF DIFFERENT DATASET SIZES!!!!!!!!!!!}

\paragraph{Selected Features for Downstream Prediction.}
Next, we trained downstrem classifiers on top of the features selected by LMPrior to evaluate their quality.
% Next, we evaluated the quality of the features selected by LMPrior by training downstream classifiers on top of them.
% In the cases where the separation of features was not completely accurate, we also conducted experiments to observe whether LMPrior could be used to select the correct features and thus increase the classification accuracy after corruption.
% Building on the dataset separation task, 
% we trained 
% classifiers on top of the features from the merged datasets which were deemed to be important by LMPrior.
% The setup was similar to Experiment 1, but we also ran simple and interpretable classifiers on the merged datasets. 
The datasets were sub-sampled so that the final sample size matched the size of the smaller dataset (typically the one being mixed in). 
% Sometimes for very small datasets, like UCI Breast Cancer and Wine, we also further reduced the dataset size by 2 in order to prevent overfitting and be able to observe a drop in the classification accuracy after corruption. 
As shown in Figure~\ref{fig:histo}, the threshold $\tau$ which completely separates the two data sources are dataset-specific---for example, the Housing and Wine datasets utilize a threshold $tau < 0.8$, while the Breast Cancer and Housing datsets use $\tau < 0.5$. We select the most appropriate threshold $\tau$ for each experiment.
% \kristy{Mention that features are selected by looking at variables whose \texttt{score}($\rvc$) exceeded some threshold $\tau$.}

We found that LMPrior selected features which increased the accuracy in classification tasks in corrupted datasets for various combinations of datasets. 
As an example, upon mixing Breast Cancer features to those of the Adult Census income dataset, the test accuracy decreased from the baseline of $89.4\%$ to $85.08\%$.
% Train/Test accuracy went down from the baseline \kristy{what exactly is the baseline here?} of 87.4\%/89.4\% to 85.9\%/85.08\%. 
Using LMPrior retained 6 breast cancer features and filtered 2 features from the income dataset (\textit{final weight, native country}). 
After filtering out the unimportant features, we recovered the original test accuracy of $89.4\%$.
% train/test classification accuracy increased back to 87.03\%/89.4\%. See Appendix for other examples. \kristy{TODO: CAREFUL}
We additionally compared our results with baselines such as LassoNet \citep{JMLR:v22:20-848}, which filter features based on their importance in the prediction based on the data. 
As shown in Figure~\ref{fig:lasso}, even when LMPrior does not achieve complete separation, it still outperforms purely data-driven feature selection.
% As can be seen in \ref{fig:lasso}, even when LMPrior doesn't segregate the feature sets completely, a common sense based feature selection still works better than data-driven feature selection. (These figures are for Cancer + Wine) (178x30 sized dataset is appended with whole of the wine dataset 178x13)
We provide additional details on the experimental setup and dataset preprocessing steps in Appendix~\ref{TODO}.\kristy{todo}

% \begin{figure}[ht!]
%   \centering
%   \includegraphics[width=2in]{figures/lasso_ftr_select.png}\\
%   \includegraphics[width=2in]{figures/gpt_ftr_select.png}\\
%   \label{fig:lasso}
% \end{figure}
\begin{figure}[!t]
    \centering
        \subfigure[housing-income]{\includegraphics[width=.45\linewidth]{figures/lasso_ftr_select.png}}
        \subfigure[housing-wine]{\includegraphics[width=.45\linewidth]{figures/gpt_ftr_select.png}}
    \caption{\kristy{FIX THIS!!!!!!!!!} \sanjari{ (These figures are for Cancer + Wine) (178x30 sized dataset is appended with whole of the wine dataset 178x13)}}
    \label{fig:lasso}
\end{figure}
% \sanjari{ In a general setting, we won't really have the feature names and descriptions so not sure about the argument we can make here.}


\subsection{Feature Selection with US Census Data}
In this experiment, we investigate a suite of real-world datasets derived from the US Census Bureau via the \texttt{folktables} API \citep{ding2021retiring}.
In particular, we leverage the Public Use Microdata Sample (PUMS) of the American Community Survey (ACS), which includes data from millions of US households each year.
% , as well as the Annual Social and Economic Supplement (ASEC) of the Current Population Survey (CPS). 
The ACS dataset is comprised of 286 numerical and categorical features such as the total number of operating vehicles owned and the total number of times that someone has moved in the past year.
We preprocess data from California households in 2018 \kristy{TODO} according to the details provided in Appendix~\ref{app-data} and predict whether an individual's commute time exceeds 20 minutes.

Our goal for this experiment is twofold. We want to not only use LMPrior to filter out nuisance variables that may hinder predictive performance, but also leverage LMPrior as a tool for \emph{exploratory data analysis} to assess which semantically meaningful features should be included. 
We compare against the following baselines: (a) 16 features (\textbf{Subset}) as in \citep{ding2021retiring}; (b) the entire dataset (\textbf{Full}); and (c) a random baseline (\textbf{Random}) which selects the same number of features returned by LMPrior.
We also consider existing feature selection baselines such as: (d) \textbf{LassoNet} \citep{JMLR:v22:20-848}. \kristy{We also demonstrate that LMPrior is complementary to existing methods [TODO]}. \kristy{TODO MORE BASELINES}
For each method, we extract the relevant features and train a Random Forest classifier with $n=100$ trees. \kristy{TODO: other methods}
% We train a RandomForest classifier with $K=100$ decision trees via \texttt{scikit-learn}, and use OpenAI's \texttt{davinci-instruct-beta} engine. We refer the reader to additional details in Appendix~\ref{TODO} for further details on the experimental setup and hyperparameter configurations. 

As shown in Table~\ref{tab:feature_selection_acs}, we find that LMPrior outperforms all baselines, selecting 59/281 features and leading to a downstream Random Forest (RF) classifier accuracy of 82.8\% at $\tau = 0$. We provide additional experimental details in Appendix~\ref{addtl-results}.
% \kristy{mention that we call threshold value $\tau$ and cut off at 0.}
% \kristy{they will probs ask for a $\tau$ ablation}
% this is with text-davinci-001
% \begin{enumerate}
%     \item Baseline with 16 features: $67\%$
%     \item Full with all 281 features (dropped 5): $74.6\%$
%     \item Random baseline with random subset of 169 features: $68.45\% \pm 0.06$ across 5 runs
%     \item LMPrior: $79.6\%$
% \end{enumerate}
% this is with davinci-instruct-beta
% \begin{enumerate}
%     \item Baseline with 16 features: $67\%$
%     \item Full with all 281 features (dropped 5): $74.6\%$
%     \item Random baseline with random subset of X features: $64.49\% \pm 0.12$ across 5 runs
%     \item LMPrior: $82.82\%$ with 59 features
% \end{enumerate}

% lassonet gets 63.07 with 59 features, and 67.9 with 425 features purely as a method. if we use it for feature selection, we get TODO.
% random also got 62.93 +- 0.09 across 10 runs
\begin{table}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
    \Xhline{\arrayrulewidth}
    &\multicolumn{1}{c}{Random Forest}
    &\multicolumn{1}{c}{Logistic Regression}&\multicolumn{1}{c}{SVM}\\
    % \cline{2-7}
    \Xhline{\arrayrulewidth}
     Subset (16) & 0.67 & - & -\\
     Full (281) & 0.75 & - & - \\
     Random (59) & 0.65  & - & -\\
     LassoNet \citep{JMLR:v22:20-848} & 0.68  & - & - \\
     LMPrior (59)  & \textbf{0.83}  & - & - \\
    \Xhline{\arrayrulewidth}
    \end{tabular}
    }
    \caption{Classifier accuracies. Higher is better. LMPrior outperforms all baselines.}
    \label{tab:feature_selection_acs}
\end{table}

% \begin{figure*}[!t]
% \centering
%      \subfigure[width=\textwidth]{figures/davinci_instruct_beta_census_california_logits.png}
%      \begin{subfigure}\includegraphics[width=\textwidth]{figures/gpt_rf_census_ca_feature_importances.png}
%      \end{subfigure}
% \caption{(Left) \kristy{TODO} Difference in logit values returned by LMPrior for \texttt{T} and \texttt{F}. \kristy{consistency with Y/N}. We threshold at $\tau=0$ to decide whether or not to include a particular feature. (Right) \kristy{TODO what is going on w fontsize} Top 10 most important features returned by the RF classifier, using features that were selected by LMPrior.}
% \label{fig:gpt_census}
% \end{figure*}

\begin{figure*}[!t]
    \centering
        \subfigure[housing-income]{\includegraphics[width=.47\textwidth]{figures/davinci_instruct_beta_census_california_logits.png}}
        \subfigure[housing-wine]{\includegraphics[width=.47\textwidth]{figures/gpt_rf_census_ca_feature_importances.png}}
    \caption{(Left) \kristy{TODO} Difference in logit values returned by LMPrior for \texttt{T} and \texttt{F}. \kristy{consistency with Y/N}. We threshold at $\tau=0$ to decide whether or not to include a particular feature. (Right) \kristy{TODO what is going on w fontsize} Top 10 most important features returned by the RF classifier, using features that were selected by LMPrior.}
    \label{fig:gpt_census}
\end{figure*}

% \begin{figure}[!t]
%     \centering
%         \includegraphics[width=\linewidth]{figures/davinci_instruct_beta_census_california_logits.png}
%     \caption{\kristy{TODO} Difference in logit values returned by LMPrior for \texttt{T} and \texttt{F}. \kristy{consistency with Y/N}. We threshold at $\tau=0$ to decide whether or not to include a particular feature.}
%     \label{fig:logit_diff}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%         \includegraphics[width=\linewidth]{figures/gpt_rf_census_ca_feature_importances.png}
%     \caption{\kristy{TODO what is going on w fontsize} Top 10 most important features returned by the RF classifier, using features that were selected by LMPrior.}
%     \label{fig:imp_features}
% \end{figure}
The important features are: wage, total earnings, total income, age, usual hours worked per week past 12 months, income-to-poverty ratio, means of transportation to work, time of departure for work, time of arrival at work, vehicle occupancy.
% \kristy{probs want the same figure but directly from LMPrior}
% \begin{figure}[!t]
%     \centering
%         \includegraphics[width=\linewidth]{figures/gpt_rf_census_ca_confidence_logits.png}
%     \caption{\kristy{TODO what is going on w fontsize} Top 10 most confident features (define confident) returned by LMPrior}
%     \label{fig:imp_features}
% \end{figure}
% Features are: occupation, age, wage, total amount of income someone has made, whether the person has worked last year, employment status, primary field of degree, "Medicare, for people 65 and older, or people with certain disabilities", industry

\subsection{Safe Reinforcement Learning}
% \paragraph{Gridworld}
In this experiment, we test the efficacy of the safe RL LMPrior \({\cal P}_\text{SRL}\) in a safety-relevant environment. We apply the LMPrior to the Island Navigation task from the AI Safety Gridworlds \cite{leike2017ai} suite. In objective of this task is to learn the optimal policy to reach the goal, while minimizing the number of safety violations, defined as instances where the agent enters a water-filled square. Since the agent is not given negative reward for entering the water squares, a training method that discourages the agent from entering the water must have some common-sense knowledge that entering the water is unwise. To extract this knowledge, we use the following prompt:

\texttt{This is a series of judgments about decisions of a navigation robot. The robot is not waterproof.}

We follow this by several proposed actions and judgments specified as \texttt{Good}, \texttt{Neutral}, or \texttt{Bad}. We use the provided feature giving the distance of the robot from the water, and textually classify it either as \texttt{in}, \texttt{close to}, \texttt{neither close nor far from}, or \texttt{far from} water. The prompt then elicits an answer as to whether the action to move to the relevant square is good, bad or neutral. We then assign the value \(1\) to \texttt{good}, \(0\) to \texttt{neutral}, and \(-1\) to \texttt{neutral}. Taking the numerical expectation of the judgments then gives us the reward to add, respectively \((-1, -0.3, 0.6, 0.95)\) for the four possible distances. We then train a PPO \cite{schulman2017proximal} agent for 100,000 steps on the environment, with and without reward shaping. We use the stable baselines \cite{raffin2019stable} implementation with default hyperparameters and repeat the experiment over ten random seeds. 

\begin{figure}[h!]
  \centering
  \includegraphics[width=2in]{figures/island-navigation.pdf}\\
  \label{fig:gridworld}
  \caption{The Island Navigation gridworld. \cc{Can put in appendix if space}}
\end{figure}

% \paragraph{Gridworld Results}
Both with and without reward shaping, we observe the policy converges to the optimal policy. 
For the environment without reward shaping, we observe \(21137 \pm 1130\) safety violations during training for the non-reward-shaped policy, and \(\textbf{4355} \pm 223\) safety violations for the reward-shaped policy, a significant reduction.

% \paragraph{Safety Gym}
% In this experiment, we test on a more challenging continuous control environment, the \texttt{Safexp-PointGoal1} environment from the Safety Gym\footnote{\url{https://openai.com/blog/safety-gym/}}. The aim of the environment is to test constrained reinforcement learning algorithms which can reach the goal without traversing hazards (depicted as blue circles). We use the same prompt as in the Island Navigation task, computing the distance to the hazard with the lidar observation. We discretize the maximum value of the hazard lidar field into a series of written descriptions similar to the Island Navigation task, and compute the expected value predicted by the language model, which we add to the reward. We then train a PPO \cite{schulman2017proximal} agent for 5,000,000 steps on the environment, with and without reward shaping. We use the stable baselines \cite{raffin2019stable} implementation with hyperparameters taken from the safety gym provided agents.

% \paragraph{Safety Gym Results}

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=2in]{figures/safety-gym.pdf}\\
%   \label{fig:gridworld}
%   \caption{The PointGoal1 environment. \cc{Can put in appendix if space, or make into double small fig with island gridworld}}
% \end{figure}


\subsection{Causal Discovery}
\paragraph{Setting.}
In this series of experiments, we show that we can combine LMPriors with data-driven methods to increase overall accuracy on a challenging causal inference task. In particular, we consider the Tuebingen Cause-Effect Pairs dataset \citep{mooij2016distinguishing}. In this dataset, a series of datasets of \((\rvx, y)\) pairs are given, along with a textual description of what \(\rvx\) and \(y\) represent. The goal is to conclude whether the causal relationship between the variables is \(\rvx \to y\), or \(y \to \rvx\). The pairs are gathered from a mix of several datasets, with \((\rvx, y)\) pairs as diverse as \texttt{(fine aggregate, compressive strength)} and \texttt{(Bytes sent, Open http connections)}. As our data-driven method, we use the RECI algorithm \cite{blobaum2018cause}, as implemented in the Causal Discovery Toolbox\footnote{\url{https://fentechsolutions.github.io/CausalDiscoveryToolbox/}}. We standardize the metadata provided in the dataset, collating a \texttt{name} and \texttt{description} for each of \(\rvx\) and \(y\), and a \texttt{brief context} for the source dataset. As is standard practice \citep{wu2020causal} we remove several pairs with either multidimensional \(\rvx, y\) or missing values. 

As described in Section~\ref{method} we incorporate the causal discovery LMPrior \({\cal P}_\text{CD}\) by constructing a prior that elicits prior probability judgments consistent with common-sense reasoning. Similarly to previous work \citep{zhao2021calibrate,liu2021makes}, we found that the design of the prompt was crucial for eliciting reasonable probability judgments. The inclusion of the explanation ensures that the context has examples of thoughtful reasoning. It can also serve as a useful tool to understand erroneous predictions, as it indicates some amount of reasoning behind the prediction. Our prompt is then shown as in Figure~\ref{fig:causal_prompt}:
% \cc{Prompt box!}
\begin{figure}[H]
  \centering
  \includegraphics[width=\linewidth]{figures/causal_prompt.png}
    \label{fig:causal_prompt}
    \caption{\kristy{TODO: mockup, this can be better. needs fixing}}
\end{figure}
% \texttt{This is a set of causal relationship facts.\\
% A -> B means that A directly causes B.\\
% The description explains why.}
We then give several examples of hypothetical \(\rvx, y\) pairs along with descriptions, context and judgment. The full prompt and experimental details are given in the appendix, \cc{appendix section} We keep the format of the judgment consistently with a \texttt{$\to$}. This means we can evaluate the model's log likelihood ratio with \(\log \lm(\rvx \vert \rvc) - \log \lm(y \vert \rvc)\). The output of RECI is a ``causal coefficient'' \(\rho \in [-1, 1]\) with \(\rho=1 \implies \rvx \to y, \rho=-1 \implies y \to \rvx\), which we interpret probabilistically as \(p(\rvx \to y) = (\rho + 1)/2\).

\paragraph{Results.}
We find that the RECI algorithm alone does not perform particularly well, detecting the correct causal direction with an accuracy of 58.7\%. The LMPrior alone does much better, achieving an accuracy of 83.5\%, consistent with high scores of language models on common-sense reasoning tasks \cc{cite}. When we combine the log-probabilities as described above, we obtain an accuracy of 84.5\%, better than either of the components alone. To our knowledge, this is higher than the current state-of-the-art performance (83.3\%)\cite{wu2020causal} of a purely data-driven algorithm applied to the data. 
This illustrates that even when combined with a weak model, the LMPrior is able to increase performance. \cc{kind of weak end there}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/universal.tex <==
\section{Language Models as Universal Priors}
\subsection{What is a language model?}
Here we will assume that a ``language model'' is a black-box function that takes in a sequence of words \((\rvx_1, \ldots, \rvx_i)\) and returns \(p(\rvx_{i+1}|\rvx_{1:i})\), or returns a sample \(\rvx_{i+1}|\rvx_{1:i}\). Since the best language models are currently proprietary\footnote{This is changing quite quickly though, so maybe we can rethink this assumption} we assume we don't have access to any of the internal statistics of the language model, and can't fine-tune it.

\subsection{Use Cases}

Pretrained LMs can be used in a variety of ways:
\begin{enumerate}
\item to \textit{score} the outputs of final generations, such as causal structures or text to quanitfy how ``realistic" or "plausible" our generations are:
  \begin{enumerate}
  \item For example, on a captioning task the language model can evaluate \texttt{The dog is reading a book} as a much less likely sentence than \texttt{The dog is eating from a bowl}. 
  \end{enumerate}
    \item to steer intermediate generations at each time step towards a desired outcome (e.g. according to a certain target).
    \item TODO
\end{enumerate}
\text{}\\
One very simple way or incorporating such pretrained LMs into a sequential prediction/generation task is by upweighting/downweighting the output logits of a classifier via the pretrained LM probabilities:
\[
p(\rvx_i|\rvx_{1:i-1}, c) \propto \plm(c|\rvx_{1:i}) p(\rvx_i|\rvx_{1:i-1})
\]
where $p_{\textrm{LM}}(c|\rvx_{1:i})$ denotes the output of a pretrained LM and $c$ is an auxiliary label denoting how likely or unlikely the entire sequence would be. 
\kristy{NOTE: this may require some fine-tuning for $\plm$?} Although this reweighting procedure is quite simple via an auxiliary attribute/domain classifier \citep{yang2021fudge}, a more natural way to incorporate such ``common sense" knowledge is to directly leverage the pretrained LM as the reweighting function.

% One very simple way or incorporating such pretrained LMs into a structured prediction task is by upweighting/downweighting the output logits of a classifier:
% \[
% p(y|\rvx, c) \propto p_{\textrm{LM}}(c|\rvx, y) p(y|\rvx)
% \]
% where $p_{\textrm{LM}}(c|\rvx, y)$ denotes the output of a pretrained LM. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

